Rejection via Learning Density Ratios

Classification with rejection emerges as a learning paradigm which allows models to abstain from making predictions. The predominant approach is to alter the supervised learning pipeline by augmenting typical loss functions, letting model rejection incur a lower loss than an incorrect prediction. Instead, we propose a different distributional perspective, where we seek to find an idealized data distribution which maximizes a pretrained model's performance. This can be formalized via the optimization of a loss's risk with a $\varphi$-divergence regularization term. Through this idealized distribution, a rejection decision can be made by utilizing the density ratio between this distribution and the data distribution. We focus on the setting where our $\varphi$-divergences are specified by the family of $\alpha$-divergence. Our framework is tested empirically over clean and noisy datasets.

==> figures/algorithm.tex <==
\begin{algorithm}[t]
\caption{\color{red} NAMETODO(\( \lambda_{c}, \gamma, \meas{P} \))}
\begin{algorithmic}[1] \label{algo:fbde}
\STATE \textbf{input}: ;
\STATE \( \meas{Q}_{1} \gets \meas{Unif} \)
\FOR{$t = 1,\ldots,T$}
    \STATE Sample mini-batch of \( b \) examples \( \{(x_{i}, y_{i})\}_{i=1}^{b} \)
    \STATE Update
\ENDFOR
\STATE \textbf{return}: $\meas{Q}_T$
\end{algorithmic}
\end{algorithm}


==> figures/phi_div_gen_table.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c c c}
        Name & \( \phi \) & \( \phi^{\star} \) & \( \grad \phi^{\star} \) \\
        KL & \( x \log x \) & \( \phi^{\star} \) & \( \grad \phi^{\star} \) \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/gradient-approximation.tex <==
\section{Gradient Based Approximation}

Although ideally we would like to utilize the optimal distributions given in the prior section, in practice there can be a number of problems. Firstly, for the general \( \varphi \) divergence, find the appropriate Lagrange multipliers can be difficult, \eg, \cref{thm:opt_amicable_dist}. Furthermore, one should note that \( [\grad_{\meas{Q}} L(\meas{Q}_{t})](x) = \expect_{\meas{P}_{\rm y \mid x}}[\ell(\Y, h(x)))]\) is required to evaluated at \( x \) to determine whether or not rejection can occur. This can be problematic as if the training data we are using to define \( \meas{Q} \) does not contain examples of \( x_{\rm test} \) in the test set, we cannot evaluate \( \meas{Q}(x_{\rm test}) \).

%Although finding the optimal adversarial rejection distribution as per \cref{thm:opt_adv}, as per the previous section, the process of solving the optimization exactly can be difficult. One alternative is to restrict the family of distribution we consider to those parameterized by a particular parameterization \( \{ \meas{Q}_{\vartheta} \in \mathcal{D}(\mathcal{X}) : \vartheta \in \vartheta \} \). This can be particularly appealing as \( \meas{Q}_{\vartheta} \) can be designed in a way such that sampling, normalization, and properties such as non-negativity are baked into the parameterized family of distributions.

As such, we propose to restrict the set of distributions we consider to learn the adversarial rejection distributions to that specified by a parameteric family of distributions \( \{ \meas{Q}_{\vartheta} \in \mathcal{D}(\mathcal{X}) : \vartheta \in \vartheta \} \). This can be particularly appealing as \( \meas{Q}_{\vartheta} \) can be designed in a way such that sampling, normalization, and properties such as non-negativity are baked into the parameterized family of distributions.

From a practical perspective, this reduces the learning of the adversarial rejection distribution to learning the parameters \( \vartheta \), which can be optimized via, \eg, gradient descent methods. As such, one can find adversarial rejection distribution of this kind by simply calculating the gradient of the optimization problem in, \eg, \cref{eq:fixed_lambda} \wrt \( \vartheta \).
%
In this case, the central object of concern is the \emph{gradient} of our updates, such that \( \meas{Q}_{\vartheta} \) can be computed via gradient descent for efficient updates.

\begin{theorem}
    \label{thm:adv_grad}
    Suppose the adversarial rejection distributions being optimized in \cref{eq:fixed_lambda} (for general \( \varphi \)-divergence) are restricted to the parmeterized set of distributions \( \{ \meas{Q}_{\vartheta} \in \mathcal{D}(\mathcal{X}) : \vartheta \in \vartheta \} \). Then the gradient of \cref{eq:fixed_lambda} \wrt \( \vartheta \) is given by,
    %
    \begin{equation}
        \label{eq:grad_update_1}
        %\expect_{\meas{P}}\left[ \frac{\meas{Q}_{\vartheta}}{\meas{P}} \cdot \grad_{\vartheta} \log \meas{Q}_{\vartheta} \cdot \left(\frac{\rho}{1+\rho} \cdot \varphi^{\prime}\left( \frac{\meas{Q}_{\vartheta}}{\meas{P}} \right) + \frac{1}{1+\rho} \cdot \varphi^{\prime}\left( \frac{\meas{Q}_{\vartheta}}{\meas{Q}_{t}} \right) + \frac{2\gamma}{1+\rho} \cdot \grad_{\meas{Q}}(L(\meas{Q})) \right) \right].
        \expect_{\meas{P}_{\rm x, \rm y}}\left[ \frac{\meas{Q}_{\vartheta}(\X)}{\meas{P}(\X)} \cdot \grad_{\vartheta} \log \meas{Q}_{\vartheta}(\X) \cdot \left( \varphi^{\prime}\left( \frac{\meas{Q}_{\vartheta}(\X)}{\meas{P}(\X)} \right) + \lambda \cdot \ell(\Y, h(\X)) \right) \right].
    \end{equation}
\end{theorem}

One should note that \cref{eq:grad_update_1} leads to an algorithm for finding \( \meas{Q}_{\vartheta} \): one can use gradient descent to optimize \cref{eq:fixed_lambda} via its gradients. The outer expectation of \cref{eq:grad_update_1} can be approximated via samples of \( \meas{P}_{\rm x, \rm y} \). However, one might notice that the gradient update requires explicit access to the distribution \( \meas{P} \) which in many domains is difficult to obtain.

% One interesting aspect is that the \( \varphi^{\prime} \) terms can be combined to be just \wrt to a single un-normalized distribution, as per \cref{eq:avg_step}.

As such, we look at a particular family of parameteric distributions inspired by \cref{thm:opt_adv}. That is, we suppose that \( \meas{Q}_{\vartheta}(x) \propto \meas{P}(x) \cdot \pi_{\vartheta}(x) \) where \( \pi_{\vartheta} \) is non-negative. This provides a number of conveniences for implementation. Notably, the exact density of \( \meas{P} \) does not to be known explicitly as long as we have enough samples. This is elucidated by the following corollary.
%
\begin{corollary}
    Suppose the conditions of \cref{thm:adv_grad} hold with \( \meas{Q}_{\vartheta}(x) \propto \meas{P}(x) \cdot \pi_{\vartheta}(x) \). Then the gradient of \cref{eq:fixed_lambda} \wrt \( \vartheta \) is given by,
    \begin{equation}
        \label{eq:grad_update_2}
        \expect_{\meas{P}_{\rm x, \rm y}}\left[ \frac{\meas{\pi}_{\vartheta}(\X)}{Z_{\vartheta}} \cdot \grad_{\vartheta} \log \left( \frac{\meas{\pi}_{\vartheta}(\X)}{Z_{\vartheta}} \right) \cdot \left( \varphi^{\prime}\left( \frac{\meas{\pi}_{\vartheta}(\X)}{Z_{\vartheta}} \right) + \lambda \cdot \ell(\Y, h(\X)) \right) \right],
    \end{equation}
    where \( Z_{\vartheta} = \expect_{\meas{P}}[\pi_{\vartheta}(\X)] \) is the normalization term of \( \meas{Q}_{\theta} \).
    %and \( \grad_{\vartheta} \log \meas{Q}_{\vartheta}(x) \) can be simplified as,
    %
    %\begin{equation}
    %    \grad_{\vartheta} \log \meas{Q}_{\vartheta}(x)
    %    =
    %    \grad_{\vartheta} \log \pi_{\vartheta}(x) - \grad_{\vartheta} \log \expect_{\meas{P}}[\pi_{\vartheta}(\X)].
    %\end{equation}
\end{corollary}

It should be noted that \( Z_{\vartheta} \) in practice will need to be approximated. However, also note that it \emph{only} requires unlabelled samples from \( \meas{P} \in \mathcal{D}(\mathcal{X}) \); and thus can be made separate from sampling approximations of the expectation of \( \meas{P}_{\rm x, \rm y} \). In practice one could approximate the samples of \( \meas{P} \) via a generative model to generate more points for the approximation of \( Z_{\vartheta} \).

Although the parametric form of \( \meas{Q}_{\theta} \) may seem to be restrictive by including \( \meas{P} \) into it, for the purposes of rejection via \cref{def:ratio_rej} it is actually a convenience. Indeed, the functional-form of the distributions simplifies the rejection function to be,
%
\begin{equation}
    r_{\tau}(x) = \lriver{\pi_{\vartheta} \leq \tau \cdot Z_{\vartheta}},
\end{equation}
which is now independent of \( \meas{P} \) and only dependent on the learnable component of \( \meas{Q}_{\vartheta} \).
In fact, given a fixed parameterization \( \vartheta \) of \( \meas{Q}_{\vartheta} \) we can take \( Z_{\vartheta} \) to be constant. That is, we ignore \( Z_{\vartheta} \) in the rejection decision and instead `tune' the combined threshold \( \tau^{\prime} = \tau \cdot Z_{\vartheta} \) \wrt the rate of rejection. In practice this can be done by taking a validation set and building a cumulative distribution of rejections \wrt \( \tau^{\prime} \).

It should be noted that in practice we want to design \( \pi_{\vartheta} \) such that it will resemble the closed form solution for a given \( \varphi \)-divergence. For instance, if \( \phi \)-divergence is specified to be the KL-divergence, we may want to specify \( \pi_{\vartheta}(x) = \exp(- \textrm{NN}_{\vartheta}(x)) \) as per \cref{eq:opt_kl_adv}; and if an \( \alpha \)-divergence is chosen we may want to leverage \cref{thm:opt_amicable_dist,cor:pos_alpha,cor:neg_alpha}.
